Localization Is All You Evaluate: Data Leakage in Online Mapping Datasets and How to Fix It

The task of online mapping is to predict a local map using current sensor observations, e.g. from lidar and camera, without relying on a pre-built map. State-of-the-art methods are based on supervised learning and are trained predominantly using two datasets: nuScenes and Argoverse 2. However, these datasets revisit the same geographic locations across training, validation, and test sets. Specifically, over $80$% of nuScenes and $40$% of Argoverse 2 validation and test samples are less than $5$ m from a training sample. At test time, the methods are thus evaluated more on how well they localize within a memorized implicit map built from the training data than on extrapolating to unseen locations. Naturally, this data leakage causes inflated performance numbers and we propose geographically disjoint data splits to reveal the true performance in unseen environments. Experimental results show that methods perform considerably worse, some dropping more than $45$ mAP, when trained and evaluated on proper data splits. Additionally, a reassessment of prior design choices reveals diverging conclusions from those based on the original split. Notably, the impact of lifting methods and the support from auxiliary tasks (e.g., depth supervision) on performance appears less substantial or follows a different trajectory than previously perceived. Splits can be found at https://github.com/LiljaAdam/geographical-splits

==> sec/all_figures.tex <==
\begin{figure*}[tb]
  \centering
   \includegraphics[width=\linewidth, trim={1mm, 0, 1mm, 0}, clip]{sec/figures/singapore-onenorth-zoom.png}
   \caption{Substantial geographical overlap between train, val, and test sets for nuscenes' singapore one north}
   \label{fig:onecol}
\end{figure*}

\begin{figure*}[tb]
  \centering
   \includegraphics[width=\linewidth, trim={1mm, 0, 1mm, 0}, clip]{sec/figures/singapore-onenorth-qualitative-examples.png}
   \caption{Qualitative example from train, val, and test sets [of NuScenes?].}
   \label{fig:onecol}
\end{figure*}

\begin{figure*}[tb]
  \centering
   \includegraphics[width=\linewidth, trim={1mm, 0, 1mm, 0}, clip]{sec/figures/instagram-example-prediction-validation.png}
   \caption{Qualitative example from InstaGRAM on validation example. Faulty ground truth is predicted well.}
   \label{fig:onecol}
\end{figure*}

\begin{figure*}[tb]
  \centering
   \includegraphics[width=\linewidth, trim={1mm, 0, 1mm, 0}, clip]{sec/figures/maptr-example-prediction-validation.png}
   \caption{Qualitative example from MapTR on validation example. Faulty ground truth is predicted well. Opaque lines are predictions, faded lines are ground truth.}
   \label{fig:onecol}
\end{figure*}

\begin{figure*}
  \centering
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=\linewidth, trim={1mm, 0, 1mm, 0}, clip]{sec/figures/argo_qual_image_example/train_315968375849927219.jpg}
    \caption{Train}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=\linewidth, trim={1mm, 0, 1mm, 0}, clip]{sec/figures/argo_qual_image_example/val_315967271949927208.jpg}
    \caption{Val}
    \label{fig:short-b}
  \end{subfigure}
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=\linewidth, trim={1mm, 0, 1mm, 0}, clip]{sec/figures/argo_qual_image_example/test_315971041399927216.jpg}
    \caption{Test}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example from argoverse [what does this explain]}
  \label{fig:short}
\end{figure*}



==> sec/tables/eval_on_closest.tex <==
\begin{table}
\small
\centering
\setlength{\tabcolsep}{2pt} % Default value: 6pt
\scalebox{0.8}{%
\caption{Evaluating the predictions from validation and test sets against the ground truth of the closest train sample. It can be seen that the performance (IoU for HDMapNet, and mAP for MapTRv2 and VectorMapNet) is lower when evaluating with the Swapped ground truth, compared to using the Real ground truth, indicating the models learn to interpolate between train samples.}
\begin{tabular}{cccc}\hline 
\toprule 
Model & Set & Real GT & Swapped GT \\ \midrule 
\multirow{2}{*}{HDMapNet} & Val  & 31.3 & 20.8 \\ 
                           & Test & 38.8 & 25.8 \\ \cmidrule{2-4} 
\multirow{2}{*}{VectorMapNet} & Val  &  43.2 & 26.4\\
                               & Test &  54.8 & 39.8 \\ \cmidrule{2-4} 
\multirow{2}{*}{MapTRv2} & Val  & 61.5 & 33.4 \\
                          & Test & 72.7 & 46.4\\ 
\bottomrule 
\end{tabular}}
\label{tab:eval-on-closest}
\end{table}


==> sec/tables/splits_table.tex <==
\begin{table}
    \centering
    \setlength{\tabcolsep}{2pt} 
    \scalebox{0.9}{%
    \begin{tabular}{@{}ccccc@{}}\hline
        \toprule 
        \multirow{2}{*}{Split} & \multirow{2}{*}{Sampling} & \multicolumn{3}{c}{\#Samples}   \\%& \multicolumn{3}{c}{Map Properties} & \multirow{2}{*}{Methods}\\ 
        \cmidrule(lr){3-5} %\cmidrule(lr){8-10}
        & & Train & Val & Test \\%& Clss & 3D & ??\\
        \midrule
        \multirow{2}{*}{Orig.} & Sparse &$28$k&$6$k&$6$k     \\
                               & Dense  &$134$k&$29$k&$26$k  \\ \cmidrule{2-5} % &  & \xmark& - \\
        \multirow{2}{*}{Geo.}  & Sparse &$28$k&$6$k&$6$k     \\ 
                               & Dense  &$130$k&$30$k&$29$k  \\ % &  & \xmark& - \\
        %\oursplitname.-Argo2 & Argo2 \cite{argoverse2_2021}  &$110$k&$24$k&$24$k\\% &  & \cmark & - \\
        \bottomrule 
    \end{tabular}}

    \caption{Number of samples in nuScenes for Original (Orig.) and Geographical (Geo.) splits. The count for sparse sampling only includes the key-frame samples, while the dense sampling also includes intermediate samples.}
    \label{tab:splits}
\end{table}
